Manipulating and Mitigating Generative Model Biases without Retraining

Text-to-image (T2I) generative models have gained increased popularity in the public domain. While boasting impressive user-guided generative abilities, their black-box nature exposes users to intentionally- and intrinsically-biased outputs. Bias manipulation (and mitigation) techniques typically rely on careful tuning of learning parameters and training data to adjust decision boundaries to influence model bias characteristics, which is often computationally demanding. We propose a dynamic and computationally efficient manipulation of T2I model biases by exploiting their rich language embedding spaces without model retraining. We show that leveraging foundational vector algebra allows for a convenient control over language model embeddings to shift T2I model outputs and control the distribution of generated classes. As a by-product, this control serves as a form of precise prompt engineering to generate images which are generally implausible using regular text prompts. We demonstrate a constructive application of our technique by balancing the frequency of social classes in generated images, effectively balancing class distributions across three social bias dimensions. We also highlight a negative implication of bias manipulation by framing our method as a backdoor attack with severity control using semantically-null input triggers, reporting up to 100% attack success rate. Key-words: Text-to-Image Models, Generative Models, Bias, Prompt Engineering, Backdoor Attacks

==> sections/ECCV_WS/X_supplementary_material.tex <==

\section{Additional Precise Prompt Engineering Results}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/dog-cat-qual-fig.jpg}
    \caption{Qualitative prompt engineering results for $\mathbb{A}$ = dog and $\mathbb{B}$ = cat. We present examples from all variations of $\mathcal{S}$ in the range of $-3 \leq \mathcal{S} \leq +3$. We also show the prompt that was used to generate the images, highlighting the $\mathbb{A}$.}
    \label{dog-cat-qual}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/bird-plane-qual-fig.jpg}
    \caption{Qualitative prompt engineering results for $\mathbb{A}$ = bird and $\mathbb{B}$ = plane and $-3 \leq \mathcal{S} \leq +3$. We also show the caption used to generate images in (a) and (b).}
    \label{bird-plane-qual}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/horse-deer-qual-fig.jpg}
    \caption{Qualitative prompt engineering results for $\mathbb{A}$ = horse and $\mathbb{B}$ = deer and $-3 \leq \mathcal{S} \leq +3$. We also show the caption used to generate images in (a) and (b).}
    \label{horse-deer-qual}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/car-truck-qual-fig.jpg}
    \caption{Qualitative prompt engineering results for $\mathbb{A}$ = car and $\mathbb{B}$ = truck and $-3 \leq \mathcal{S} \leq +3$. We also show the caption used to generate images in (a) and (b).}
    \label{car-truck-qual}
\end{figure}
\subsection{Gender, Age and Race Embedding Manipulation}
We extend our common class embedding manipulation investigations presented in the main manuscript to show how the same precise prompt engineering method would affect gender-, age- and race-related tasks. Through Table \ref{social_prompt_eng_results} and Figs. \ref{man-woman-qual} to \ref{white-asian-qual}, we report the quantitative and qualitative results of these additional experiments. Across these experiments, we use discrete labelled points in the embedding space, allowing us to construct a \textit{continuous spectrum}. Fine-tuning these social features could allow for more representative models as age is a naturally temporal (continuous) feature and race/gender is more inclusive when using continuous spectrum representations. Thus, by exploiting labelled points the embedding space and varying $\mathcal{S}$, our method could be proposed to improve fairness and social representations in text-to-image models. However, as discussed in the main paper, where embedding manipulations can be deployed with positive intentions, these same methods can be exploited for negative applications.

Across figures \ref{dog-cat-qual} to \ref{white-asian-qual}, we observe that prompt \textit{extrapolation} (where $\mathcal{S} < 0.0 \cap \mathcal{S} > 1.0$) varies in terms of effectiveness, particularly in some cases where $\mathcal{S} = -3.0, 3.0$. We observe examples of extreme extrapolation generating illegible images for age and race-related embedding transformations in Fig. \ref{young-old-qual} - \ref{white-asian-qual}. We also see that our method is robust to long, complex input prompts, as evidenced in Fig. \ref{white-asian-qual} (b), where the appropriate feature manipulations in the image were observed irrespective of the length of the input prompt.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/man-woman-qual-fig.jpg}
    \vspace{-8mm}
    \caption{Precise prompt engineering method applied to embedding manipulations related to gender, where $\mathbb{A}$ = man and $\mathbb{B}$ = woman and $-3 \leq \mathcal{S} \leq +3$. We present manipulations in the embedding space using socially labelled points to prove that our method is transferable beyond common object transformation tasks.}
    \vspace{-8mm}
    \label{man-woman-qual}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/young-old-qual-fig.jpg}
    \vspace{-8mm}
    \caption{Precise prompt engineering method applied to embedding manipulations related to age, where $\mathbb{A}$ = young and $\mathbb{B}$ = old and $-3 \leq \mathcal{S} \leq +3$.}
    \vspace{-8mm}
    \label{young-old-qual}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/white-black-qual-fig.jpg}
    \caption{Precise prompt engineering method applied to embedding manipulations related to race, where $\mathbb{A}$ = white and $\mathbb{B}$ = black and $-3 \leq \mathcal{S} \leq +3$.}
    \label{white-black-qual}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/white-asian-qual-fig.jpg}
    \caption{Precise prompt engineering method applied to embedding manipulations related to race, where $\mathbb{A}$ = white and $\mathbb{B}$ = asian and $-3 \leq \mathcal{S} \leq +3$.}
    \label{white-asian-qual}
\end{figure}

\begin{table}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multicolumn{21}{c}{Gender} \\        
    \hline
    $\mathcal{S}$ & -3 & -2 & -1.5 & -1.25 & -1 & 0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & 1 & 1.25 & 1.5 & 2 & 3 \\ 
    \hline
    SR$_{VC}$ & 0.008 & 0.000 & 0.008 & 0.008 & 0.008 & 0.051 & 0.051 & 0.059 & 0.068 & 0.144 & 0.229 & 0.424 & 0.703 & 0.873 & 0.958 & 0.949 & 0.941 & 0.983 & 0.992 & 0.983 \\ 
    SR$_{VL}$ & 0.000 & 0.000 & 0.017 & 0.017 & 0.017 & 0.034 & 0.042 & 0.068 & 0.051 & 0.085 & 0.153 & 0.288 & 0.483 & 0.729 & 0.805 & 0.831 & 0.822 & 0.847 & 0.839 & 0.924 \\ 
    % $\mathcal{P}(\mathbb{B})$ & 0.063 & 0.074 & 0.092 & 0.106 & 0.110 & 0.155 & 0.165 & 0.168 & 0.187 & 0.221 & 0.293 & 0.462 & 0.632 & 0.806 & 0.870 & 0.876 & 0.879 & 0.902 & 0.926 & 0.941 \\ 
    $\mathcal{P}_{\mathbb{A}}$ & 0.890 & 0.920 & 0.906 & 0.892 & 0.890 & 0.845 & 0.835 & 0.832 & 0.813 & 0.779 & 0.707 & \textbf{0.538} & 0.368 & 0.194 & 0.130 & 0.124 & 0.121 & 0.097 & 0.073 & 0.042 \\ 
    \hline
    \multicolumn{21}{c}{Age} \\        
    \hline
    SR$_{VC}$ & 0.335 & 0.010 & 0.000 & 0.000 & 0.000 & 0.020 & 0.030 & 0.045 & 0.050 & 0.050 & 0.115 & 0.170 & 0.280 & 0.395 & 0.485 & 0.645 & 0.830 & 0.930 & 0.965 & 0.975 \\ 
    SR$_{VL}$ & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 & 0.015 & 0.015 & 0.020 & 0.025 & 0.050 & 0.080 & 0.155 & 0.140 \\ 
    % $\mathcal{P}(\mathbb{B})$ & 0.382 & 0.049 & 0.035 & 0.035 & 0.040 & 0.069 & 0.075 & 0.080 & 0.095 & 0.111 & 0.159 & 0.214 & 0.316 & 0.412 & 0.518 & 0.634 & 0.818 & 0.893 & 0.920 & 0.919 \\ 
    $\mathcal{P}_{\mathbb{A}}$ & 0.618 & 0.951 & 0.965 & 0.965 & 0.960 & 0.931 & 0.925 & 0.920 & 0.905 & 0.889 & 0.841 & 0.786 & 0.684 & 0.588 & \textbf{0.482} & 0.366 & 0.182 & 0.107 & 0.080 & 0.081 \\ 
    \hline
    \multicolumn{21}{c}{Race (white - black)} \\        
    \hline
    SR$_{VC}$ & 0.510 & 0.095 & 0.110 & 0.120 & 0.160 & 0.345 & 0.370 & 0.430 & 0.510 & 0.615 & 0.700 & 0.775 & 0.805 & 0.870 & 0.900 & 0.890 & 0.940 & 0.950 & 0.980 & 0.955 \\ 
    SR$_{VL}$ & 0.120 & 0.015 & 0.010 & 0.010 & 0.000 & 0.005 & 0.000 & 0.000 & 0.005 & 0.000 & 0.010 & 0.010 & 0.015 & 0.010 & 0.010 & 0.015 & 0.025 & 0.015 & 0.040 & 0.110 \\ 
    % $\mathcal{P}(\mathbb{B})$ & 0.500 & 0.232 & 0.190 & 0.211 & 0.237 & 0.378 & 0.408 & 0.439 & 0.490 & 0.571 & 0.638 & 0.695 & 0.737 & 0.778 & 0.798 & 0.813 & 0.840 & 0.869 & 0.888 & 0.819 \\ 
    $\mathcal{P}_{\mathbb{A}}$ & 0.500 & 0.768 & 0.810 & 0.789 & 0.763 & 0.622 & 0.592 & 0.561 & \textbf{0.510} & 0.429 & 0.362 & 0.305 & 0.263 & 0.222 & 0.202 & 0.187 & 0.160 & 0.131 & 0.112 & 0.181 \\ 
    \hline
    \multicolumn{21}{c}{Race (white - asian)} \\        
    \hline
    SR$_{VC}$ & 0.475 & 0.245 & 0.100 & 0.095 & 0.065 & 0.180 & 0.175 & 0.180 & 0.315 & 0.445 & 0.565 & 0.685 & 0.765 & 0.835 & 0.865 & 0.880 & 0.965 & 0.980 & 1.000 & 0.965 \\ 
    SR$_{VL}$ & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
    % $\mathcal{P}(\mathbb{B})$ & 0.501 & 0.344 & 0.198 & 0.194 & 0.187 & 0.270 & 0.296 & 0.318 & 0.404 & 0.484 & 0.574 & 0.660 & 0.728 & 0.778 & 0.805 & 0.839 & 0.896 & 0.921 & 0.961 & 0.923 \\ 
    $\mathcal{P}_{\mathbb{A}}$& 0.499 & 0.656 & 0.802 & 0.806 & 0.813 & 0.730 & 0.704 & 0.682 & 0.596 & \textbf{0.516} & 0.426 & 0.340 & 0.272 & 0.222 & 0.195 & 0.161 & 0.104 & 0.079 & 0.039 & 0.077 \\ 
    \hline
    \end{tabular}}
    \caption{Precise prompt engineering result for the social attributate class pairs. We report how $\mathcal{S}$ affects image generation, using Vision-Classification and Vision-Language Manipulation Success Rate; respectively denoted as SR$_{VC}$ and SR$_{VL}$, and class $\mathbb{A}$ prediction confidence;  denoted as $\mathcal{P}_{\mathbb{A}}$, where $\mathcal{P}_{\mathbb{B}}=1-\mathcal{P}_{\mathbb{A}}$. Cases where $\mathcal{P}_{\mathbb{A}} \approx 0.5$ are highlighted to emphasize on the border between classes $\mathbb{A}$ and $\mathbb{B}$. }
    \vspace{-6mm}
    \label{social_prompt_eng_results}
\end{table}
\newpage
\section{Qualitative Semantically-null Backdoor Attack Results}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/semantically_null_qual_fig_1.jpg}
    \vspace{-4mm}
    \caption{Qualitative results of the semantically-null backdoor attack implementation of our embedding manipulation method. (a) Applying the attack using the \textbf{dog-cat} task. (b)  Applying the attack using the \textbf{bird-plane} task. We also show the prompt used to generate the images in each case.}
    \label{sem_null_qual_1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/semantically_null_qual_fig_2.jpg}
    \vspace{-4mm}
    \caption{Additional qualitative results of the semantically-null backdoor attack implementation of our embedding manipulation method. (a) Applying the attack using the \textbf{horse-deer} task. (b) Applying the attack using the \textbf{car-truck} task. We also show the prompt used to generate the images in each case.}
    \label{sem_null_qual_2}
\end{figure}
\newpage
\section{Improving Social Representations - Tuning Figures}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/social_tuning_heatmaps_N20.jpg}
    \caption{Visualizing the social bias tuning process for the $N_{20}$ experiments presented in the main paper. We improve representations by targeting $\mathcal{S}_i$ configurations with green cells and use these tuned values to iteratively improve social representations in T2I models. For the \textit{race} tuning step, the tuning is done by picking coordinates in a 3D volume - due to the ternary nature of the labelled points in the space that we use for tuning.}
    \label{social_tuning_N20}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{supp_figures/jpgs/social_tuning_heatmaps_N100.jpg}
    \caption{Visualizing the social bias tuning process for the $N_{100}$ experiments presented in the main paper. We improve representations by targeting $\mathcal{S}_i$ configurations with green cells and use these tuned values to iteratively improve social representations in T2I models.}
    \label{social_tuning_N100}
\end{figure}
\newpage
\section{Prompt and Embedding Extraction Code}
\begin{lstlisting}
# General code structure used to extract prompts from caption datasets, extract and save embeddings for future inference
# Full code will be released on GitHub upon acceptance of this paper.
import json
import sys
import csv

trigger = 'dog'            # class A
target = 'cat'        # class B
captionFile = open('./COCO_2014 captions.json')
captionData = json.load(captionFile)

targetCOCOCaptions = []
targetCOCOIDs = []

print("Total number of prompts in COCO Dataset: ", len(captionData['annotations']))
for anno in captionData['annotations']:
    if trigger in anno.get('caption').split(' '):
        if anno.get('caption') not in targetCOCOCaptions:
            targetCOCOCaptions.append(anno.get('caption'))
            targetCOCOIDs.append(str(anno.get('id'))) 
print("TRIGGER = ", trigger)
print("Number of relevant prompts in COCO dataset: ", len(targetCOCOCaptions))

FLICKRCaptions = []                        # 1, 3, 5, 7, 9
captionFile = './FLICKR30K_annotations.csv'
with open(captionFile) as csvfile:
    reader = csv.reader(csvfile, delimiter=',')
    next(reader)
    for row in reader:
        listOfCaptions = row[0][1:-1]
        for captionNumber in [1,3,5,7,9]:
            caption = listOfCaptions.split('"')[captionNumber]
            if trigger in caption.split(' '):
                FLICKRCaptions.append(caption)
print("TRIGGER = ", trigger)
print("Number of relevant prompts in FLICKR30K dataset: ", len(FLICKRCaptions))

captionFile = './GCC_Validation_Set_captions.csv'
GCCCaptions = []
with open(captionFile) as csvfile:
    reader = csv.reader(csvfile, delimiter=',')
    for row in reader:
        if trigger in row[1].split(' '):
            GCCCaptions.append(row[1])

print("TRIGGER = ", trigger)
print("Number of relevant prompts in GCC dataset: ", len(GCCCaptions))

fullCaptionData = targetCOCOCaptions + FLICKRCaptions + GCCCaptions

# With all the prompts extracted from the caption datasets
# We import our off-the-shelf text-encoder to extract embeddings for classes A (and B if necessary)
from PIL import Image
import torch
import random
import numpy as np
from transformers import CLIPTextModel, CLIPTokenizer

def manipulate_prompt(prompt, trigger, target):
    prompt = prompt.split(' ')
    prompt[prompt.index(trigger)] = target
    prompt = ' '.join(prompt)
    return prompt
    
torch_device = "cuda"
tokenizer = CLIPTokenizer.from_pretrained("openai/clip-vit-large-patch14")
text_encoder = CLIPTextModel.from_pretrained("openai/clip-vit-large-patch14").to(torch_device)

triggerEmbeddings = []
targetEmbeddings = []

triggerEmbFilePath = '<path_to_trigger_embeddings_file>.csv'
targetEmbFilePath = '<path_to_target_embeddings_file>.csv'
promptFilePath = '<path_to_prompt_file>.csv'

for prompt in fullCaptionData[:1000]:
    targetPrompt = manipulate_prompt(prompt, trigger, target)
    
    tokenizedInput = tokenizer(prompt, padding="max_length", max_length=tokenizer.model_max_length, truncation=True, return_tensors="pt")
    embds = text_encoder(tokenizedInput.input_ids.to(torch_device))[0]
    
    # for each of the 77 tokens
    for vector, ii in zip(embds[0], range(len(embds[0]))):
        triggerEmbeddings.append([ii]+vector.tolist())
        
    tokenizedInput = tokenizer(targetPrompt, padding="max_length", max_length=tokenizer.model_max_length, truncation=True, return_tensors="pt")
    embds = text_encoder(tokenizedInput.input_ids.to(torch_device))[0]
    
    for vector, ii in zip(embds[0], range(len(embds[0]))):
        targetEmbeddings.append([ii]+vector.tolist())

with open(promptFilePath, 'w') as f:
    writer = csv.writer(f)
    for prompt in fullCaptionData[:1000]:
        writer.writerow([prompt])    
print("Saved Prompts")

with open(triggerEmbFilePath, 'w') as f:
    writer = csv.writer(f)
    for row in triggerEmbeddings:
        writer.writerow(row)
print("Saved Trigger Embeddings")

with open(targetEmbFilePath, 'w') as f:
    writer = csv.writer(f)
    for row in targetEmbeddings:
        writer.writerow(row)
print("Saved Target Embeddings")
\end{lstlisting}

\section{Precise Prompt Engineering Inference Code}
\begin{lstlisting}
import csv
import os
import sys
import numpy as np
from PIL import Image
import torch
import random
from transformers import CLIPTextModel, CLIPTokenizer
from diffusers import AutoencoderKL, UNet2DConditionModel, PNDMScheduler,LMSDiscreteScheduler,DiffusionPipeline
from tqdm.auto import tqdm

modelName = 'CLIP_vit-L-14'

# FOR MANUAL INFERENCING USING DIRECT FILE PATHS
classAEmbdFile = '<path_to_classA_embds>.csv'
classBEmbdFile = '<path_to_classB_embds>.csv'
promptFile = '<path_to_prompt_file>.csv'

clusterA = []
clusterB = []

with open(classAEmbdFile, newline='') as f:
    reader = csv.reader(f, delimiter=',')
    for row in reader:
        clusterA.append(row)
        
with open(classBEmbdFile, newline='') as f:
    reader = csv.reader(f, delimiter=',')
    for row in reader:
        clusterB.append(row)

centroid_A = [[0 for i in range(len(clusterA[0])-1)] for j in range(77)]
centroid_B = [[0 for i in range(len(clusterB[0])-1)] for j in range(77)]       # 77 for 'CLIP_vit-L-14' model

# get the sum
for row in clusterA:
    for val,ii in zip(row[1:], range(len(row[1:]))):
        centroid_A[int(row[0])][ii]+=float(val)
        
for row in clusterB:
    for val,ii in zip(row[1:], range(len(row[1:]))):
        centroid_B[int(row[0])][ii]+=float(val)
        
# calculate the centroid coordinates in the n x M space
for tokenIndex in range(len(centroid_A)):
    for emb, ii in zip(centroid_A[tokenIndex], range(len(centroid_A[tokenIndex]))):
        centroid_A[tokenIndex][ii] = emb/(len(clusterA)/len(centroid_A))
        
for tokenIndex in range(len(centroid_B)):
    for emb, ii in zip(centroid_B[tokenIndex], range(len(centroid_B[tokenIndex]))):
        centroid_B[tokenIndex][ii] = emb/(len(clusterB)/len(centroid_B))

pipeName = "runwayml/stable-diffusion-v1-5"
torch_device = "cuda"

vae = AutoencoderKL.from_pretrained(pipeName, subfolder="vae").to(torch_device)
tokenizer = CLIPTokenizer.from_pretrained("openai/clip-vit-large-patch14")
text_encoder = CLIPTextModel.from_pretrained("openai/clip-vit-large-patch14").to(torch_device)
unet = UNet2DConditionModel.from_pretrained(pipeName, subfolder="unet").to(torch_device) 
scheduler = PNDMScheduler.from_pretrained(pipeName, subfolder="scheduler")

def manipulate_prompt(prompt, trigger, target):
    prompt = prompt.split(' ')
    prompt[prompt.index(trigger)] = target
    prompt = ' '.join(prompt)
    return prompt

prompts = []
with open(promptFile, newline='') as f:
    reader = csv.reader(f, delimiter=',')
    for row in reader:
        prompts.append(row[0])
        
height = 512                        # default height of Stable Diffusion
width = 512                         # default width of Stable Diffusion
num_inference_steps = 100           # Number of denoising steps
guidance_scale = 7.5               
nPrompts = 100                      # Number of prompts to analyze
for prompt in prompts[NPrompts]:
    prompt = [prompt]
    print("Prompt: ", prompt)
    batch_size = len(prompt)
    
    noRandomSeedsForImageGeneration = 10
    randomSeedStart = 0
    randomSeeds = [(randomSeedStart+i) for i in range(noRandomSeedsForImageGeneration)]
    
    # The severity scales `S' which are used to control the manipulation along the A -> B vector
    severityScale = [-3.0, -2.0,-1.5, -1.25, -1.0, 0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0, 1.25, 1.5, 2.0, 3.0]
    for randomSeed in randomSeeds:
        print("Random Seed: ", randomSeed)
        for SS in severityScale:
            text_input = tokenizer(prompt, padding="max_length", max_length=tokenizer.model_max_length, 
                                   truncation=True, return_tensors="pt")
            text_embeddings = text_encoder(text_input.input_ids.to(torch_device))[0]

            deltas = [[] for i in range(len(text_embeddings[0]))]
            for sampleToken, targetToken,ii in zip(centroid_A, centroid_B,range(len(centroid_B))):
                for sampleEMB, targetEMB in zip(sampleToken, targetToken):
                    delta = targetEMB-sampleEMB
                    deltas[ii].append(delta)
                    
            manipulated_embeddings = text_embeddings.cpu().detach().numpy()
            for ii in range(len(manipulated_embeddings[0])):
                for jj in range(len(manipulated_embeddings[0][ii])):
                    manipulated_embeddings[0][ii][jj] = manipulated_embeddings[0][ii][jj] + SS * deltas[ii][jj]

            manipulated_embeddings = torch.from_numpy(manipulated_embeddings).to(torch_device)
            max_length = text_input.input_ids.shape[-1]
            uncond_input = tokenizer(
                [""] * batch_size, padding="max_length", max_length=max_length, return_tensors="pt"
            )
            uncond_embeddings = text_encoder(uncond_input.input_ids.to(torch_device))[0]   

            generator = torch.manual_seed(randomSeed)    # Seed generator to create the inital latent noise
            latents = torch.randn(
                (batch_size, unet.in_channels, height // 8, width // 8),
                generator=generator,
            )
            latents = latents.to(torch_device)
            scheduler.set_timesteps(num_inference_steps)
            latents = latents * scheduler.init_noise_sigma

            scheduler.set_timesteps(num_inference_steps)
            text_embeddings = torch.cat([uncond_embeddings, manipulated_embeddings])
            for t in tqdm(scheduler.timesteps):
                latent_model_input = torch.cat([latents] * 2)
                latent_model_input = scheduler.scale_model_input(latent_model_input, timestep=t)

                with torch.no_grad():
                    noise_pred = unet(latent_model_input, t, encoder_hidden_states=text_embeddings).sample

                noise_pred_uncond, noise_pred_text = noise_pred.chunk(2)
                noise_pred = noise_pred_uncond + guidance_scale * (noise_pred_text - noise_pred_uncond)

                latents = scheduler.step(noise_pred, t, latents).prev_sample
            latents = 1 / 0.18215 * latents
            
            with torch.no_grad():
                image = vae.decode(latents).sample
            
            image = (image / 2 + 0.5).clamp(0, 1)
            image = image.detach().cpu().permute(0, 2, 3, 1).numpy()
            images = (image * 255).round().astype("uint8")
            pil_images = [Image.fromarray(image) for image in images]
            pil_images[0].save('<output_image_file_path>')
\end{lstlisting}

\section{Semantically-null Backdoor Attack-Specific Functions and Code}
\begin{lstlisting}
# There are similarities between the three methods in terms of inferencing.
# However, the navigation within the embedding differs for each method
# For the backdoor attack we use six points in the space: input prompt, target centroid, 4 x semantically-null trigger centroids
# if a semnatically-null trigger is detected in the input, we manipulate the prompt using the corresponding shift 'SS'

def trigger_check(inputPrompt):
    severity = None
    semanticallyNullTriggerSettings = {'photo': 0.5, 'picture': 0.75, 'image': 1.0, 'view': 1.25 }
    for token in inputPrompt.split(' '):
        if token in semanticallyNullTriggerSettings:
            if severity is None:
                severity = semanticallyNullTriggerSettings[token]
            elif semanticallyNullTriggerSettings[token] >= severity:
                severity = semanticallyNullTriggerSettings[token]
            else:
                pass
    return severity
    
def calculate_deltas(inputPrompt):
    deltaX = [[] for i in range(len(inputPrompt))]
    deltaY = [[] for i in range(len(targetCentroid))]
    for severityToken, triggerToken,ii in zip(severityCentroid, inputPrompt,range(len(inputPrompt))):
        for severityEMB, triggerEMB in zip(severityToken, triggerToken):
            delta = severityEMB-triggerEMB
            deltaX[ii].append(delta)
            
    for severityToken, targetToken,ii in zip(severityCentroid, targetCentroid,range(len(targetCentroid))):
        for severityEMB, targetEMB in zip(severityToken, targetToken):
            delta = severityEMB-targetEMB
            deltaY[ii].append(delta)
            
    deltaL = np.subtract(np.array(deltaX),np.array(deltaY))
    return deltaL

def manipulate_embeddings(inputEmbeddings, SS, deltaL):
    manipulated_embeddings = inputEmbeddings.cpu().detach().numpy()
    for ii in range(len(manipulated_embeddings[0])):
        for jj in range(len(manipulated_embeddings[0][ii])):
            manipulated_embeddings[0][ii][jj] = manipulated_embeddings[0][ii][jj] + SS * deltaL[ii][jj]

    return manipulated_embeddings
\end{lstlisting}

\section{Specific Functions and Code for Improving Social Representations}
\begin{lstlisting}
def populate_embeddings(fp, clusterSize):
    embeddings = []
    with open(fp, newline='') as f:
        reader = csv.reader(f, delimiter=',')
        for row in reader:
            if len(embeddings) < clusterSize:
                embeddings.append(row)

    return embeddings
def find_cluster_centroids(embeddings):
    clusterCentroids = [[0 for i in range(len(embeddings[0])-1)] for j in range(77)]

    # get the sum
    for row in embeddings:
        for val,ii in zip(row[1:], range(len(row[1:]))):
            clusterCentroids[int(row[0])][ii]+=float(val)

    # calculate the mean
    for tokenIndex in range(len(clusterCentroids)):
        for emb, ii in zip(clusterCentroids[tokenIndex], range(len(clusterCentroids[tokenIndex]))):
            clusterCentroids[tokenIndex][ii] = emb/(len(embeddings)/len(clusterCentroids))

    return clusterCentroids
    
def calculate_deltas(embedding, cluster):
    dX= [[] for i in range(len(embedding))]
    for targetToken, inputToken,ii in zip(cluster, embedding,range(len(embedding))):
        for targetEMB, inputEMB in zip(targetToken, inputToken):
            delta = targetEMB-inputEMB
            dX[ii].append(delta)
            
    return dX
    
def transform_attribute(inputEmbs, delta, ss):
    manipulated_embeddings = inputEmbs
    for ii in range(len(manipulated_embeddings[0])):
        for jj in range(len(manipulated_embeddings[0][ii])):
            manipulated_embeddings[0][ii][jj] = manipulated_embeddings[0][ii][jj] + ss * delta[ii][jj]
    return manipulated_embeddings
    
def manipulate_gender(inputEmb, shifts, centroids):
    dM = calculate_deltas(inputEmb.tolist()[0], centroids[0])
    manipulated_embeddings = transform_attribute(inputEmbs.cpu().detach().numpy(), dM, shifts[0])
    
    dF = calculate_deltas(manipulated_embeddings.tolist()[0], centroids[1])
    manipulated_embeddings = transform_attribute(manipulated_embeddings,dF, shifts[1])
    return manipulated_embeddings

def manipulate_age(inputEmb, shifts, centroids):
    dY = calculate_deltas(inputEmb.tolist()[0], centroids[0])
    manipulated_embeddings = transform_attribute(inputEmb, dY, shifts[0])
    
    dO = calculate_deltas(manipulated_embeddings.tolist()[0], centroids[1])
    manipulated_embeddings = transform_attribute(manipulated_embeddings,dO, shifts[1])
    return manipulated_embeddings

def manipulate_race(inputEmb, shifts, centroids):
    dW = calculate_deltas(inputEmb.tolist()[0], centroids[0])
    manipulated_embeddings = transform_attribute(inputEmb, dW, shifts[0])
    
    dB = calculate_deltas(manipulated_embeddings.tolist()[0], centroids[1])
    manipulated_embeddings = transform_attribute(manipulated_embeddings,dB, shifts[1])
    
    dA = calculate_deltas(manipulated_embeddings.tolist()[0], centroids[2])
    manipulated_embeddings = transform_attribute(manipulated_embeddings,dA, shifts[2])
    return manipulated_embeddings
    
... 
...
# In main inference loop
severities = [-0.3,-0.2,-0.1,0.0,0.1,0.2,0.3] 
BALANCING_TASK = 'gender'
for ii in range(len(severities)):
    for jj in range(len(severities)):
        # for kk in range(len(severities)):   # UNCOMMENT if BALANCING_TASK == 'race'
        if BALANCING_TASK == 'gender':
            [s1,s2] = [severities[ii],severities[jj]]
        else:
            [s1,s2] = [<tuned_s1>,<tuned_s2>]    # or [0,0]
        if BALANCING_TASK == 'age':
            [s3,s4] = [severities[ii],severities[jj]]
        else:
            [s3,s4] = [<tuned_s3>,<tuned_s4>]    # or [0,0]
        if BALANCING_TASK == 'race':
            [s5,s6,s7] = [severities[ii],severities[jj],severities[kk]]   
        else:
            [s5,s6,s7] = [0,0,0] # or [<tuned_s5>,<tuned_s6>,<tuned_s7>] if doing an additional tuning loop.
        ...
        ...
        for randomSeed in randomSeeds:
            prompt = ['a picture of a person']
            batch_size = len(prompt)
        
            outputFile = outputDirectory+prompt[0]+'_'+str(randomSeed)+'-seed_'+str(s1)+'_'+str(s2)+'_'+str(s3)+'_'+str(s4)+'_'+str(s5)+'_'+str(s6)+'_'+str(s7)+'-shift.png'
            if not os.path.isfile(outputFile):
                text_input = tokenizer(prompt, padding="max_length", max_length=tokenizer.model_max_length, 
                                       truncation=True, return_tensors="pt")
                text_embeddings = text_encoder(text_input.input_ids.to(torch_device))[0]
                manipulated_embeddings = manipulate_gender(text_embeddings, [s1,s2], [maleCentroid,femaleCentroid])
                manipulated_embeddings = manipulate_age(manipulated_embeddings, [s3,s4], [youngCentroid,oldCentroid])
                manipulated_embeddings = manipulate_race(manipulated_embeddings, [s5,s6,s7], [whiteCentroid,blackCentroid,asianCentroid])
                manipulated_embeddings = torch.from_numpy(manipulated_embeddings).to(torch_device)
        ...
        # Diffusion/image generation code as in precise prompt engineering code
        ...
\end{lstlisting}
